BETA: Binarized Energy-Efficient Transformer Accelerator at the Edge

Existing binary Transformers are promising in edge deployment due to their compact model size, low computational complexity, and considerable inference accuracy. However, deploying binary Transformers faces challenges on prior processors due to inefficient execution of quantized matrix multiplication (QMM) and the energy consumption overhead caused by multi-precision activations. To tackle the challenges above, we first develop a computation flow abstraction method for binary Transformers to improve QMM execution efficiency by optimizing the computation order. Furthermore, a binarized energy-efficient Transformer accelerator, namely BETA, is proposed to boost the efficient deployment at the edge. Notably, BETA features a configurable QMM engine, accommodating diverse activation precisions of binary Transformers and offering high-parallelism and high-speed for QMMs with impressive energy efficiency. Experimental results evaluated on ZCU102 FPGA show BETA achieves an average energy efficiency of 174 GOPS/W, which is 1.76~21.92x higher than prior FPGA-based accelerators, showing BETA's good potential for edge Transformer acceleration.

==> 5-concls-r1.tex <==
\section{Conclusion}\label{sec:concls}
\Rone{In this paper, we propose a configurable open-source posit dot-product unit (PDPU) capable of performing efficient dot-product operations in deep learning applications.}
% \Rone{PDPU, equipped with a balanced 6-stage pipeline, achieves excellent area and power efficiency by leveraging fused and mixed-precision techniques.}
\Rone{PDPU features a balanced 6-stage pipeline with fused and mixed-precision properties, achieving excellent area and power efficiency.}
\Rone{Moreover, a configurable PDPU generator is developed to support diverse computational needs for deep learning applications.}
% It provides higher computational performance and hardware efficiency, benefiting from fused and mixed-precision arithmetic.
% The capability of supporting arbitrary posit formats, dot-product size and alignment width allows PDPU to be embedded as computing unit for various DNNs.
% A fine-grained 6-stage pipelined is also proposed to further improve the thoughput of PDPU.
Compared to the existing conventional dot-product hardware implementation, PDPU achieves a significant reduction of 43\%, 60\%, and 70\% in terms of area, latency, and power, respectively.
% , showing its great potential for deep learning applications.
